Online Harassment in Majority Contexts: Examining Harms and Remedies across Countries

Online harassment is a global problem. This article examines perceptions of harm and preferences for remedies associated with online harassment with nearly 4000 participants in 14 countries around the world. The countries in this work reflect a range of identities and values, with a focus on those outside of North American and European contexts. Results show that perceptions of harm are higher among participants from all countries studied compared to the United States. Non-consensual sharing of sexual photos is consistently rated as harmful in all countries, while insults and rumors are perceived as more harmful in non-U.S. countries, especially harm to family reputation. Lower trust in other people and lower trust in sense of safety in one's neighborhood correlate with increased perceptions of harm of online harassment. In terms of remedies, participants in most countries prefer monetary compensation, apologies, and publicly revealing offender's identities compared to the U.S. Social media platform design and policy must consider regional values and norms, which may depart from U.S. centric-approaches.

==> charts.tex <==
\begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{BanningbyCountry.png}
  \caption{Preferences for remedies by remedy type (top) and country (bottom).}
  \Description{sdfsdf}
  \label{figure:remedyplots}
\end{figure}

\begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{RemovingbyCountry.png}
  \caption{Preferences for remedies by remedy type (top) and country (bottom).}
  \Description{sdfsdf}
  \label{figure:remedyplots}
\end{figure}

\begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{LabelingbyCountry.png}
  \caption{Preferences for remedies by remedy type (top) and country (bottom).}
  \Description{sdfsdf}
  \label{figure:remedyplots}
\end{figure}

\begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{PaymentbyCountry.png}
  \caption{Preferences for remedies by remedy type (top) and country (bottom).}
  \Description{sdfsdf}
  \label{figure:remedyplots}
\end{figure}

\begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{RatingbyCountry.png}
  \caption{Preferences for remedies by remedy type (top) and country (bottom).}
  \Description{sdfsdf}
  \label{figure:remedyplots}
\end{figure}

\begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{ApologybyCountry.png}
  \caption{Preferences for remedies by remedy type (top) and country (bottom).}
  \Description{sdfsdf}
  \label{figure:remedyplots}
\end{figure}

\begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{RevealingbyCountry.png}
  \caption{Preferences for remedies by remedy type (top) and country (bottom).}
  \Description{sdfsdf}
  \label{figure:remedyplots}
\end{figure}


%CHARTS IN FORMATTED LAYOUT
\begin{figure}
    \centering
    {\includegraphics[width=0.5\textwidth]{SexualHarassmentbyCountry.png}} 
    {\includegraphics[width=0.5\textwidth]{PsychologicalbyCountry.png}} 
    {\includegraphics[width=0.5\textwidth]{SafetybyCountry.png}}
    {\includegraphics[width=0.5\textwidth]{ReputationbyCountry.png}}
    \caption{Perceptions of harm by harm type: (a) Sexual Harassment (b) Psychological Harm (c) Physical Safety (d) Family Reputation}
    \label{fig:HarmbyHarmType}
\end{figure}
